StructBoost: Boosting Methods for Predicting Structured Output Variables

Boosting is a method for learning a single accurate predictor by linearly combining a set of less accurate weak learners. Recently, structured learning has found many applications in computer vision. Inspired by structured support vector machines (SSVM), here we propose a new boosting algorithm for structured output prediction, which we refer to as StructBoost. StructBoost supports nonlinear structured learning by combining a set of weak structured learners. As SSVM generalizes SVM, our StructBoost generalizes standard boosting approaches such as AdaBoost, or LPBoost to structured learning. The resulting optimization problem of StructBoost is more challenging than SSVM in the sense that it may involve exponentially many variables and constraints. In contrast, for SSVM one usually has an exponential number of constraints and a cutting-plane method is used. In order to efficiently solve StructBoost, we formulate an equivalent $ 1 $-slack formulation and solve it using a combination of cutting planes and column generation. We show the versatility and usefulness of StructBoost on a range of problems such as optimizing the tree loss for hierarchical multi-class classification, optimizing the Pascal overlap criterion for robust visual tracking and learning conditional random field parameters for image segmentation.

==> bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]
{author_fig/Chunhua_Shen.jpg}}]{Chunhua Shen}
is an Associate Professor at School of Computer Science, The University of Adelaide.
Prior to that, he was with the computer vision
program at NICTA (National ICT Australia), Canberra Research
Laboratory for over five years. His research interests are in the
intersection of computer vision and statistical machine learning.
Recent work has been on real-time object detection, large-scale image
retrieval and classification, and scalable nonlinear optimization.

He studied at Nanjing University, at Australian National University,
and received his PhD degree from University of Adelaide. In 2012,
he was awarded the Australian Research Council Future Fellowship.
\end{IEEEbiography}



 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_fig/Guosheng_Lin_gray.jpg}}]{Guosheng Lin}
 is a PhD candidate at School of Computer Science, The University of
 Adelaide.
 His research interests are on computer vision and machine learning.
 He received a Bachelor degree and a Master degree from the
 South China University of Technology in computer science in 2007 and 2010 respectively.
 \end{IEEEbiography}


 \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_fig/Anton_gray.jpg}}]{Anton van~den~Hengel}
 is the founding Director of The Australian Centre for Visual Technologies (ACVT).
 He is a Professor in  School of Computer Science,
 The University of Adelaide. He received a PhD in Computer Vision in 2000,
 a Masters Degree in Computer Science in 1994,
 a Bachelor of Laws in 1993, and a Bachelor of Mathematical Science in 1991, all from
 The University of Adelaide.
 \end{IEEEbiography}
%
%
%

